Bayesian optimization of a free-electron laser

The Linac Coherent Light Source changes configurations multiple times per day, necessitating fast tuning strategies to reduce setup time for successive experiments. To this end, we employ a Bayesian approach to transport optics tuning to optimize groups of quadrupole magnets. We use a Gaussian process to provide a probabilistic model of the machine response with respect to control parameters from a modest number of samples. Subsequent samples are selected during optimization using a statistical test combining the model prediction and uncertainty. The model parameters are fit from archived scans, and correlations between devices are added from a simple beam transport model. The result is a sample-efficient optimization routine, which we show significantly outperforms existing optimizers.

==> macros.tex <==
% The following approach actually works for typesetting non-italic Greek letters
\DeclareMathVersion{mathchartertext}
\SetSymbolFont{letters}{mathchartertext}{OML}{mdbch}{m}{n}
\newcommand{\gchar}[1]{\mathversion{mathchartertext}$#1$\mathversion{normal}}
% The \gchar{\char} can be used in text to type. Charter non-italic Greek characters. Usage example: \gchar{\phi}. From: http://www.khirevich.com/latex/font/

\DeclareMathVersion{mathchartertext}
\SetSymbolFont{letters}{mathchartertext}{OML}{mdbch}{m}{n}
\newcommand{\charmu}{\mathversion{mathchartertext}$\mu$\mathversion{normal}}
% \charmu is used in text to type Greek "mu",
% resulting in Charter non-italic "mu" 
% From: http://www.khirevich.com/latex/font/

% The following helps to stack lines within a table cell
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
%http://tex.stackexchange.com/questions/2441/how-to-add-a-forced-line-break-inside-a-table-cell

%\newcommand{\sgn}[1]{$\,\mathrm{sgn}#1\,$}

%\newcommand{\sign}[1]{$\frac{#1}{\abs{#1}$}

\def\erf{\operatorname{erf}}
\def\avg#1{\left\langle #1 \right\rangle}


\def\variance#1{\left\langle(#1-\left\langle#1\reft\rangle)^2\right\rangle}

\def\degree{^{\circ}}
\def\deg{^{\circ}}


%\newcommand{\um}{\gchar{\mu}m\,}
%\newcommand{\oneum}{1~\gchar{\mu}m\,}
\newcommand{\um}{\charmu m\,}
\newcommand{\oneum}{1 \charmu m\,}


%_______________________________________
% the following is from http://web.engr.illinois.edu/~jeffe/pubs/tex/jeffe.sty

% ---- SYMBOLS ----
\let\e\varepsilon               % a ``real'' epsilon

%\def\Integer{\mathsf{Z\hspace{-0.4em}Z}}
%\def\Natural{\mathrm{I\!N}}
%\def\Real{\mathrm{I\!R}}
%\def\Proj{\mathrm{I\!P}}		% projective space
%\def\Hyper{\mathrm{I\!H}}	% hyperbolic space
%
%%
%%  These two look okay in Computer Modern 11pt, or Concrete Roman
%%  12pt, but they need serious work in other sizes.  I need to figure
%%  out how to draw a vertical bar, or better yet a shallow arc, inside
%%  the bowls.  Or maybe I need to learn METAFONT.  Or maybe I should just
%%  hold my nose and use \mathbb.
%%
%\def\Complex{\mathrm{\,\raise 0.33ex\hbox{\scriptsize\bf(}\!\!\!C}}
%\def\Rational{\mathrm{\,\raise 0.33ex\hbox{\scriptsize\bf(}\!\!\!Q}}

%
%  I give up.  These are in the wrong font, but my kludged versions 
%  LOOK like kludges, especially \Z, \Q, and \C.
%
\def\Real{\mathbb{R}}
\def\Proj{\mathbb{P}}
\def\Hyper{\mathbb{H}}
\def\Integer{\mathbb{Z}}
\def\Natural{\mathbb{N}}
\def\Complex{\mathbb{C}}
\def\Rational{\mathbb{Q}}

\let\N\Natural
\let\Q\Rational
\let\R\Real
\let\Z\Integer
\def\Rd{\Real^d}
\def\RP{\Real\Proj}
\def\CP{\Complex\Proj}

% ---- OPERATORS (requires amsmath) ----
\def\aff{\operatorname{aff}}		
\def\area{\operatorname{area}}
\def\argmax{\operatornamewithlimits{arg\,max}}
\def\argmin{\operatornamewithlimits{arg\,min}}
\def\Aut{\operatorname{Aut}}		% Automorphism group
\def\card{\operatorname{card}}	% cardinality, deprecated for \abs
\def\conv{\operatorname{conv}}	
\def\E{\operatorname{E}}			% Expectation: $\E[X]$ (like \Pr)
\def\EE{\operatornamewithlimits{E}}
\def\Hom{\operatorname{Hom}}		% Homomorphism group
\def\id{\operatorname{id}}		% identity
\def\im{\operatorname{im}}		% image
\def\lcm{\operatorname{lcm}}
\def\lfs{\operatorname{lfs}}		% local feature size
\def\poly{\operatorname{poly}}
\def\polylog{\operatorname{polylog}}
\def\rank{\operatorname{rank}}
\def\rel{\operatorname{rel\,}}	% relative (interior, boundary, etc.)
\def\sgn{\operatorname{sgn}}
\def\vol{\operatorname{vol}}		% volume

\def\fp#1{^{\underline{#1}}}		% falling powers: $n\fp{d}$
\def\rp#1{^{\overline{#1}}}		% rising powers:  $n\rp{d}$


% --- Darts and fences ---
% less nice replacements for stmaryrd characters
%\@ifundefined{shortrightarrow}{\let\shortrightarrow\rightarrow}{}
%\@ifundefined{shortleftarrow}{\let\shortleftarrow\leftarrow}{}
%\@ifundefined{shortuparrow}{\let\shortuparrow\uparrow}{}
%\@ifundefined{shortdownarrow}{\let\shortdownarrow\downarrow}{}

\def\arcto{\mathord\shortrightarrow}
\def\arc#1#2{#1\arcto#2}
\def\cra#1#2{#1\mathord\shortleftarrow#2}
\def\fence#1#2{#1\mathord\shortuparrow#2}
\def\ecnef#1#2{#1\mathord\shortdownarrow#2}

% --- Cheap displaystyle operators ---
\def\Frac#1#2{{\displaystyle\frac{#1}{#2}}}
\def\Sum{\sum\limits}
\def\Prod{\prod\limits}
\def\Union{\bigcup\limits}
\def\Inter{\bigcap\limits}
\def\Lor{\bigvee\limits}
\def\Land{\bigwedge\limits}
\def\Lim{\lim\limits}
\def\Max{\max\limits}
\def\Min{\min\limits}

% ---- RELATORS ----
\def\deq{\stackrel{\scriptscriptstyle\triangle}{=}}	% Use := instead.
\def\into{\DOTSB\hookrightarrow}		% = one-to-one
\def\onto{\DOTSB\twoheadrightarrow}
\def\inonto{\DOTSB\lhook\joinrel\twoheadrightarrow}
\def\from{\leftarrow}
\def\tofrom{\leftrightarrow}
\def\mapsfrom{\mathrel{\reflectbox{$\mapsto$}}}
\def\longmapsfrom{\mathrel{\reflectbox{$\longmapsto$}}}

% ---- DELIMITER PAIRS ----
\def\floor#1{\lfloor #1 \rfloor}
\def\ceil#1{\lceil #1 \rceil}
\def\seq#1{\langle #1 \rangle}
\def\set#1{\{ #1 \}}
\def\abs#1{\mathopen| #1 \mathclose|}			% use instead of $|x|$ 
\def\norm#1{\mathopen\| #1 \mathclose\|}		% use instead of $\|x\|$ 
\def\indic#1{\big[#1\big]}		% indicator variable; Iverson notation
								% e.g., Kronecker delta = [x=0]

% --- Self-scaling delmiter pairs ---
\def\Floor#1{\left\lfloor #1 \right\rfloor}
\def\Ceil#1{\left\lceil #1 \right\rceil}
\def\Seq#1{\left\langle #1 \right\rangle}
\def\Set#1{\left\{ #1 \right\}}
\def\Abs#1{\left| #1 \right|}
\def\Norm#1{\left\| #1 \right\|}
\def\Paren#1{\left( #1 \right)}		% need better macro name!
\def\Brack#1{\left[ #1 \right]}		% need better macro name!
\def\Indic#1{\left[ #1 \right]}		% indicator variable; Iverson notation
